Auditing Stealth Sycophancy in Mental-Health Dialogue: Structured Clinical-State Diagnostics and Clean Matched Benchmarks

Mental-health dialogue models are increasingly evaluated by AI-based evaluators, yet these evaluators often treat surface empathy, supportiveness, or fluency as evidence of safety. In this paper, we study a hidden failure mode that we call implicit sycophancy: a response may appear empathetic while implicitly reinforcing catastrophizing, avoidance, hopeless prediction, or CBT-style labeling. To examine this problem, we introduce a diagnostic benchmark for implicit-sycophancy detection, built from three representative mental-health dialogue sources covering everyday peer support, counseling-style emotional support, and crisis-oriented interaction, and further construct a leakage-audited clean single-response matched benchmark with 500 contexts and 1,500 matched response windows. We then propose Dynamic Emotional Signature Graphs (DESG), a structured offline audit framework that separates LLM-based state extraction from final scoring and evaluates clinical direction through semantic, affective, and cognitive-distortion state transitions rather than free-form LLM judgment. Unlike metadata, surface-style, lexical, embedding, and rubric-LLM baselines, DESG scores the direction of clinical-state change induced by a response; on the leakage-audited clean matched benchmark, DESG-StateRisk improves over the strongest non-DESG baseline by 0.0488 macro-F1 and achieves the best harmful-risk detection result. These results suggest that evaluating implicit sycophancy requires explicit clinical-state modeling together with leakage checks, shortcut controls, and competitive baselines.

==> tables/table2_feature_ablation.tex <==
\begin{table}[t]
\centering
\small
\caption{Clinical feature ablations for the ConcatANN scorer on the three-source benchmark. $\Delta$ is full ConcatANN macro-F1 minus the ablated held-out score; negative values mean the ablation improved the point estimate.}
\label{tab:feature_ablation}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lccc}
\toprule
Ablation & Macro-F1 & 95\% CI & $\Delta$ F1 \\
\midrule
semantic-only & 0.6559 & [0.6192, 0.6912] & +0.2644 \\
Mental Filter & 0.8004 & [0.7636, 0.8331] & +0.1199 \\
valence & 0.8168 & [0.7806, 0.8482] & +0.1034 \\
arousal & 0.8191 & [0.7859, 0.8539] & +0.1011 \\
Labeling & 0.8352 & [0.8012, 0.8697] & +0.0850 \\
Mind Reading & 0.8375 & [0.8037, 0.8711] & +0.0828 \\
Fortune Telling & 0.8375 & [0.8037, 0.8711] & +0.0828 \\
Should Statements & 0.8375 & [0.8037, 0.8711] & +0.0828 \\
All-or-Nothing Thinking & 0.8397 & [0.8059, 0.8739] & +0.0805 \\
Overgeneralization & 0.8397 & [0.8059, 0.8739] & +0.0805 \\
Personalization & 0.8397 & [0.8071, 0.8737] & +0.0805 \\
Emotional Reasoning & 0.8533 & [0.8205, 0.8837] & +0.0670 \\
Catastrophizing & 0.8555 & [0.8226, 0.8858] & +0.0647 \\
clinical-only & 0.8755 & [0.8454, 0.9047] & +0.0447 \\
\bottomrule
\end{tabular*}
\end{table}

==> tables/table3_case_studies.tex <==
\begin{table}[t]
\centering
\small
\caption{Deterministic case-study candidates selected from held-out disagreements. Snippets are abbreviated; interpretations are descriptive and not clinical outcome claims.}
\label{tab:case_studies}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lllll}
\toprule
Case & Gold & RubricJudge & Semantic-only & Clinical-only \\
\midrule
implicit-sycophancy & harmful & neutral & harmful & harmful \\
productive-or-neutral-contrast & productive & neutral & neutral & productive \\
\bottomrule
\end{tabular*}
\end{table}


==> tables/table_deep_branch_ablation.tex <==
\begin{table}[t]
\centering
\caption{DESG-Deep branch ablations on cached-state tune reruns.}
\label{tab:deep_branch_ablation}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}llrrrrl}
\toprule
Split & Variant & Mean & Min & Max & $\Delta$ & Status \\
\midrule
existing & deep\_default & 0.8606 & 0.8433 & 0.8734 & +0.0000 & reference \\
existing & deep\_mtp & 0.8521 & 0.8446 & 0.8594 & -0.0085 & not selected \\
existing & deep\_no\_mixup & 0.8631 & 0.8581 & 0.8715 & +0.0025 & inconclusive \\
existing & deep\_no\_contrastive & 0.8575 & 0.8355 & 0.8696 & -0.0031 & inconclusive \\
existing & deep\_fixed\_k\_1 & 0.8584 & 0.8433 & 0.8695 & -0.0022 & diagnostic \\
existing & deep\_fixed\_k\_3 & 0.8584 & 0.8433 & 0.8695 & -0.0022 & diagnostic \\
existing & deep\_fixed\_k\_5 & 0.8620 & 0.8464 & 0.8721 & +0.0014 & diagnostic \\
existing & deep\_fixed\_k\_7 & 0.8615 & 0.8464 & 0.8734 & +0.0009 & diagnostic \\
existing & deep\_fixed\_k\_9 & 0.8611 & 0.8464 & 0.8711 & +0.0005 & diagnostic \\
existing & deep\_fixed\_k\_11 & 0.8611 & 0.8464 & 0.8754 & +0.0005 & diagnostic \\
\bottomrule
\end{tabular*}
\end{table}


==> tables/table_deep_ensemble_robustness.tex <==
\begin{table}[!htbp]
\centering
\scriptsize
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{0.88}
\caption{Deep and ensemble robustness across random seeds in local cached-state reruns.}
\label{tab:deep_ensemble_robustness}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}llrrr}
\toprule
Split & Method & Mean & Min & Max \\
\midrule
Existing & ConcatANN & 0.8375 & 0.8375 & 0.8375 \\
Existing & \textsc{DESG-Deep} & 0.8606 & 0.8433 & 0.8734 \\
Existing & \textsc{DESG-Ensemble} & 0.9087 & 0.8944 & 0.9196 \\
Group & ConcatANN & 0.8306 & 0.8306 & 0.8306 \\
Group & \textsc{DESG-Deep} & 0.8681 & 0.8539 & 0.8828 \\
Group & \textsc{DESG-Ensemble} & 0.9226 & 0.9133 & 0.9286 \\
\bottomrule
\end{tabular*}
\end{table}


==> tables/table_embedding_ablation.tex <==
\begin{table}[t]
\centering
\scriptsize
\caption{Supplementary embedding-interface robustness audit. The 384-D row simulates the MiniLM-native semantic space by projecting both patient and template states to the first 384 coordinates inside the existing fixed-width scorer.}
\label{tab:embedding_ablation}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llcccl}
\toprule
Semantic variant & Method & Existing & Group & $\Delta$ & Supplement conclusion \\
\midrule
minilm\_padded\_1536 & ConcatANN & 0.8375 & 0.8306 & -- & current padded reference \\
minilm\_padded\_1536 & DESG-core & 0.7980 & 0.7932 & -- & current padded reference \\
minilm\_384\_projected & ConcatANN & 0.8329 & 0.8329 & -0.0046 & padding-insensitive within 0.01 macro-F1 \\
minilm\_384\_projected & DESG-core & 0.7932 & 0.7835 & -0.0048 & padding-insensitive within 0.01 macro-F1 \\
clinical\_only\_constant\_semantic & ConcatANN & 0.8755 & 0.8800 & 0.0381 & semantic track removed control \\
clinical\_only\_constant\_semantic & DESG-core & 0.7738 & 0.7713 & -0.0242 & semantic track removed control \\
\bottomrule
\end{tabular}
}
\end{table}


==> tables/table_evidence_map.tex <==
\begin{table}[t]
\centering
\small
\caption{Evidence map for interpreting the diagnostic benchmark. Each block states what the evidence supports and what it should not be used to claim.}
\label{tab:evidence_map}
\begin{tabularx}{\linewidth}{p{0.23\linewidth}XX}
\toprule
Evidence block & Supports & Does not support \\
\midrule
Constructed split & Cached clinical states are predictive under the reported constructed protocol & Artifact-free clinical generalization \\
Metadata/BoW audit & Benchmark-construction shortcuts are strong and must be reported & That DESG learned causal clinical structure \\
Clean matched benchmark & DESG-StateRisk outperforms metadata, lexical, surface, rubric-LLM, and text-embedding risk baselines under context-level splits & Clinical deployment validity or treatment efficacy \\
Stress-balanced set & Selected-direction stress inputs expose a boundary for cached-state template scoring & That direct judges are universally stronger across protocols \\
Qualitative cases & Surface empathy can hide harmful direction and evaluator disagreement & Statistical proof by case evidence alone \\
\bottomrule
\end{tabularx}
\end{table}


==> tables/table_failure_taxonomy.tex <==
\begin{table}[t]
\centering
\small
\caption{Diagnostic risk taxonomy exposed by the audit. The categories summarize existing experimental evidence and define how each claim is bounded.}
\label{tab:failure_taxonomy}
\begin{tabularx}{\linewidth}{p{0.24\linewidth}XX}
\toprule
Diagnostic risk & Evidence in this paper & How the claim is bounded \\
\midrule
Benchmark shortcut & Metadata-only reaches 0.9946 macro-F1 and shallow BoW remains above 0.92 on the original split & Original-split scores are reported as constructed-protocol diagnostics, not artifact-free generalization \\
Judge protocol dependence & Released evaluators and the direct judge are weak on the original split, while the direct judge keeps signal on the stress audit & We do not claim that LLM judges universally fail; evaluator behavior is protocol-dependent \\
Cached-state stress boundary & On the selected-direction stress audit, ConcatANN and \textsc{DESG-core} reach only 0.1667 and 0.2698 macro-F1 & This stress format is treated as a separate input-structure diagnostic, not as the main clean matched benchmark \\
Matched-benchmark residual lexical signal & TextEmbedding-Risk reaches 0.6006 macro-F1 on the clean matched risk task & We report embedding and BoW controls directly; DESG-StateRisk remains higher at 0.6494 \\
Label-protocol dependence & Original benchmark labels are constructed and artifact-prone, while the stress split changes which evaluator family works best & The benchmark is treated as an audit protocol, not as a finished clinical-label resource \\
\bottomrule
\end{tabularx}
\end{table}


==> tables/table_qualitative_evidence.tex <==
\begin{table}[t]
\centering
\small
\caption{Qualitative evidence map. Cases are illustrative audit examples, not standalone statistical evidence.}
\label{tab:qualitative_evidence}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llllp{0.34\linewidth}}
\toprule
Claim & Gold & Judge & ConcatANN & Example \\
\midrule
Implicit sycophancy & harmful & productive & harmful & crisis-cradle:cradle-48:seed:4:harmful:v1 \\
LLM judge blindness & harmful & productive & harmful & crisis-cradle:cradle-191:seed:4:harmful:v0 \\
Cognitive distortion reinforcement & harmful & productive & harmful & clinical-esconv:esconv-464:center:8:harmful:v1 \\
Neutral plateau vs productive reframing & productive & neutral & productive & crisis-cradle:cradle-377:seed:6:productive:v0 \\
External evaluator instability & harmful & -- & -- & clinical-esconv:esconv-104:center:23:harmful:v0 \\
\bottomrule
\end{tabular}
}
\end{table}


==> tables/table_sanity_controls.tex <==
\begin{table}[t]
\centering
\small
\caption{Mechanism sanity controls. Negative deltas indicate degradation after disrupting temporal order or clinical-state dimensions.}
\label{tab:sanity_controls}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}llcc}
\toprule
Method & Control & Macro-F1 & $\Delta$ \\
\midrule
ConcatANN & default & 0.8375 & 0.0000 \\
ConcatANN & turn\_reverse & 0.8375 & 0.0000 \\
ConcatANN & turn\_shuffle & 0.8375 & 0.0000 \\
ConcatANN & cognition\_permutation & 0.8465 & 0.0091 \\
ConcatANN & emotion\_zero & 0.9954 & 0.1579 \\
DESG-core & default & 0.7980 & 0.0000 \\
DESG-core & turn\_reverse & 0.7537 & -0.0443 \\
DESG-core & turn\_shuffle & 0.7956 & -0.0024 \\
DESG-core & cognition\_permutation & 0.8004 & 0.0024 \\
DESG-core & emotion\_zero & 0.8822 & 0.0842 \\
\bottomrule
\end{tabular*}
\end{table}


==> tables/table_stress_confusion_ci.tex <==
\begin{table*}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{2.5pt}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llrlll}
\toprule
Source & Reference & N & Macro-F1 [95\% CI] & Confusion (gold rows H/N/P) & Interpretation \\
\midrule
Direct judge & Benchmark test (36) & 36 & 0.7387 [0.5897, 0.8704] & H:12/0/0; N:0/10/2; P:0/7/5 & test-split direct signal \\
Stress-calibrated State Ridge & Benchmark test (36) & 36 & 0.4558 [0.2946, 0.6102] & H:8/2/2; N:5/3/4; P:4/2/6 & improves state scorer but remains below direct judge \\
\bottomrule
\end{tabular}
}
\caption{Stress-set confusion and bootstrap confidence intervals. H/N/P denote harmful, neutral, and productive columns inside each gold-label row. The calibrated state ridge is selected on train/dev only and evaluated on the held-out stress test split.}
\label{tab:stress_confusion_ci}
\end{table*}


==> tables/table_stress_set_model_audit.tex <==
\begin{table}[t]
\centering
\small
\caption{Supplementary stress-set model audit with rule-based heuristic states. Each window is scored against harmful, neutral, and productive expert templates, and the prediction is the highest-similarity template direction.}
\label{tab:stress_set_model_audit}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccp{0.47\linewidth}}
\toprule
Method & State source & Macro-F1 & Supplement conclusion \\
\midrule
ConcatANN & Heuristic-state & 0.1667 & boundary diagnostic; heuristic templates are not optimized for the ordinal direction cue \\
DESG-core & Heuristic-state & 0.1667 & boundary diagnostic; heuristic templates are not optimized for the ordinal direction cue \\
\bottomrule
\end{tabular}%
}
\end{table}


==> tables/table_stress_state_calibration.tex <==
\begin{table}[t]
\centering
\small
\begin{tabularx}{\linewidth}{lccX}
\toprule
Method & Dev macro-F1 & Test macro-F1 & Reading \\
\midrule
Stress-calibrated State Ridge & 0.4951 & 0.4558 & cached state features recover some stress signal after calibration, but remain well below the direct judge \\
Direct judge & -- & 0.7387 & raw-text judging is stronger on this label-origin-balanced stress split \\
\bottomrule
\end{tabularx}
\caption{Artifact-controlled state-scorer calibration on the stress split. The ridge scorer uses only the cached center-state vector, selects its ridge value on the development split, and reports held-out test performance after retraining on train+development.}
\label{tab:stress_state_calibration}
\end{table}


==> tables/table_terminology_checklist.tex <==
\begin{table}[t]
\centering
\small
\caption{Terminology used throughout the paper. These terms separate state extraction, final judging, released evaluator baselines, and diagnostic metrics.}
\label{tab:terminology_checklist}
\begin{tabularx}{\linewidth}{p{0.26\linewidth}X}
\toprule
Term & Meaning in this paper \\
\midrule
Direct LLM judge & A baseline that reads raw dialogue text and directly predicts \textit{productive}, \textit{neutral}, or \textit{harmful}. DeepSeekJudge is this direct DeepSeek-v4-pro judge. \\
External evaluator & A released evaluator checkpoint run on dialogue text, such as Prometheus-2, Praetor-7B, TRACT, or Auto-J. It is not trained on the DESG state cache. \\
Internal state-based method & A method that consumes only the frozen state cache after extraction, for example SymmetricState, ConcatANN, or DESG variants. \\
State cache & The frozen per-turn state vectors used by all internal methods: MiniLM semantic embeddings padded to the 1536-D interface plus structured affective and cognitive fields. \\
Clinical regime & One of six discrete state labels: Regulated, Numb/Withdrawn, Distressed/Ruminative, Cathartic Release, Reframing/Insight, and Cognitive Deterioration. \\
Expert template & A fixed CBT-informed prototype trajectory graph used for graph matching. Templates are programmatic prototypes, not clinician-confirmed treatment plans. \\
\(\ClinicalPrior\) & A fixed directed transition-prior matrix over clinical regimes. Positive entries penalize deterioration; negative entries allow recovery-oriented compensation; near-zero entries remain close to the base metric. \\
\(\EITE\) acceptance rate & A counterfactual fidelity-gate diagnostic reporting how often the E-ITE comparison is admissible. It is not a classifier macro-F1. \\
Specificity & Specificity of the binary harmful call against the distortion-reinforcement indicator; higher values mean fewer false harmful alarms on non-reinforcing windows. \\
Coverage & Number of held-out windows with parseable or otherwise usable outputs. Missing external-evaluator outputs are reported, not imputed. \\
\bottomrule
\end{tabularx}
\end{table}

